Challenges in Measuring Bias via Open-Ended Language Generation

Researchers have devised numerous ways to quantify social biases vested in pretrained language models. As some language models are capable of generating coherent completions given a set of textual prompts, several prompting datasets have been proposed to measure biases between social groups -- posing language generation as a way of identifying biases. In this opinion paper, we analyze how specific choices of prompt sets, metrics, automatic tools and sampling strategies affect bias results. We find out that the practice of measuring biases through text completion is prone to yielding contradicting results under different experiment settings. We additionally provide recommendations for reporting biases in open-ended language generation for a more complete outlook of biases exhibited by a given language model. Code to reproduce the results is released under https://github.com/feyzaakyurek/bias-textgen.

==> Challenges in Measuring Bias via Open-Ended Language Generation/billboard.tex <==
% Please add the following required packages to your document preamble:
\begin{table*}[!]
\caption{We recommend a reporting scheme similar to bidimensional leaderboards introduced in \citet{kasai2021bidimensional} when reporting biases. Depending on the kind of contribution; whether it is a new prompt set or a new bias metric, new rows or columns may be added to the table. In the case of a debiasing technique, the table should be repeated to show posterior effects. Human Eval should be performed on a subsample of generations. Here, we show results for GPT-3---a large Transformer-decoder only language model from which we sample 5 completions given a prompt and provide average scores. Tool \#1 and \#2 for sentiment measurements are VADER and DistilBERT, respectively. Moreover, Tool \#1 and \#2 for toxicity are detoxify library by unitaryai and \href{https://perspectiveapi.com}{Perspective API} which was developed by Jigsaw, respectively. %Similar to our analysis with GPT-2, we observe that experiment settings have significant effect on ratio of metrics.
}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clccccccc}
\hline
Prompt Set                         & \begin{tabular}[c]{@{}l@{}}Decoding Parameters\\ (temperature, tokens)\end{tabular} & Human Eval. & Regard                & \multicolumn{2}{c}{Toxicity}                & \multicolumn{2}{c}{Sentiment}               & Your Metric \\ \hline
                                   & \multicolumn{1}{l}{}                                                               &              & Tool \#1             & Tool \#1             & Tool \#2             & Tool \#1             & Tool \#2             &             \\ \midrule
\multirow{4}{*}{BOLD}              & (1.0, 10) & & 1.03 & 1.83 & 0.85 & 1.25& 0.98&\\
                                   & (1.0, 30) & & 1.04 & 1.62 & 0.83 & 1.21& 0.97 & \\
                                   & (0.6, 10) & & 1.01 & 1.60 & 0.84 & 1.19& 0.97& \\
                                   & (0.6, 30) & & 1.04 & 1.61 & 0.83 & 1.27& 0.97&             \\ \hline
\multirow{4}{*}{Nozza et al. 2020} & (1.0, 10) & & 0.99 &1.22 & 1.30 & 0.98 &1.39 &\\
                                   & (1.0, 30) & & 0.99 &1.31 & 1.29 & 1.04 &1.19 &\\
                                   & (0.6, 10) & & 1.02 &1.46 & 1.41 & 0.98 &1.17 &\\
                                   & (0.6, 30) & & 0.98 &1.88 & 1.36 & 1.07 &1.31 &\\ \hline
Your Prompt Set                    &                                                                                     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  \\
\bottomrule
\end{tabular}
}
\label{tb:billboard}
\end{table*}



